An AutoML-based approach for Network Intrusion Detection

In this paper, we present an automated machine learning (AutoML) approach for network intrusion detection, leveraging a stacked ensemble model developed using the MLJAR AutoML framework. Our methodology combines multiple machine learning algorithms, including LightGBM, CatBoost, and XGBoost, to enhance detection accuracy and robustness. By automating model selection, feature engineering, and hyperparameter tuning, our approach reduces the manual overhead typically associated with traditional machine learning methods. Extensive experimentation on the NSL-KDD dataset demonstrates that the stacked ensemble model outperforms individual models, achieving high accuracy and minimizing false positives. Our findings underscore the benefits of using AutoML for network intrusion detection, as the AutoML-driven stacked ensemble achieved the highest performance with 90\% accuracy and an 89\% F1 score, outperforming individual models like Random Forest (78\% accuracy, 78\% F1 score), XGBoost and CatBoost (both 80\% accuracy, 80\% F1 score), and LightGBM (78\% accuracy, 78\% F1 score), providing a more adaptable and efficient solution for network security applications.

==> kw3.tex <==
While ML systems offer advantages over traditional methods, ML-based approaches are considered shallow learning techniques as that rely heavily on feature engineering and manual selection \cite{wagh2013survey, garg2017novel}. These methods can struggle with processing large-scale intrusion data, which often results in lower recognition accuracy and a higher false alarm rate. In contrast, DL-based intrusion detection \cite{wang2017malware, torres2016analysis, su2020bat} bypasses the need for manual feature selection and can directly process raw traffic data, improving accuracy and scalability.


In this paper, we present a comparative study on the adaptation of machine learning and deep learning methods to build Network Intrusion Detection systems. By examining both approaches, we aim to address the limitations of ML-based NID systems and explore how DL techniques can enhance detection capabilities and system performance. The contributions of this comparative study are as follows:


To overcome these issues, AutoML-based approaches \cite{salehin2024automl} have emerged as a powerful alternative as they eliminate the need for manual feature selection and can directly process raw traffic data, resulting in improved scalability and accuracy. Furthermore, AutoML enhances interpretability through the integration of explainable AI (XAI) techniques, addressing the need for transparency in complex ML models.
